A Note on the Convergence of Denoising Diffusion Probabilistic Models

Diffusion models are one of the most important families of deep generative models. In this note, we derive a quantitative upper bound on the Wasserstein distance between the data-generating distribution and the distribution learned by a diffusion model. Unlike previous works in this field, our result does not make assumptions on the learned score function. Moreover, our bound holds for arbitrary data-generating distributions on bounded instance spaces, even those without a density w.r.t. the Lebesgue measure, and the upper bound does not suffer from exponential dependencies. Our main result builds upon the recent work of Mbacke et al. (2023) and our proofs are elementary.

==> my-macros.tex <==

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{hyperref}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{natbib}

\usepackage{tikz}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environnement deriv pour les derivations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newlength{\indentationFormule} 
\setlength{\indentationFormule}{1.3em}
\newlength{\indentationTotaleFormule}
\newlength{\indentationCommentaire}
\setlength{\indentationCommentaire}{4em}
\newlength{\indentationDerivation}
\newlength{\largeurLangle}
\settowidth{\largeurLangle}{$\langle$\hspace*{.4em}}
\newlength{\largeurBoiteCommentaire}
%\newlength{\predboxwidth}
%\newlength{\savebaselineskip}
%\newlength{\derivationskip}


%\makeatletter
%\newcommand{\@indenteFormule}{\hspace*{\indentationFormule}}
\newenvironment{deriv}[1][\leftmargini]%
{\setlength{\indentationDerivation}{#1}%
\setlength{\indentationTotaleFormule}{\indentationFormule}
\addtolength{\indentationTotaleFormule}{#1}
\setlength{\largeurBoiteCommentaire}{\linewidth}
\addtolength{\largeurBoiteCommentaire}{-\indentationFormule}
\addtolength{\largeurBoiteCommentaire}{-\indentationCommentaire}
\addtolength{\largeurBoiteCommentaire}{-\largeurLangle}
\addtolength{\largeurBoiteCommentaire}{-\indentationDerivation}
\begin{list}{}{\setlength{\leftmargin}{\indentationTotaleFormule}}
\setlength{\baselineskip}{2.3\baselineskip}
\item$}%
{\hbox{}$\end{list}}  % \hbox{} evite des erfull lors d'usages
% sans \< et sans \commentaire (et avec
% des \\ pour changer de ligne).
%    \trivlist\item\relax\let\>\@indenteFormule\leftskip\indentationTotaleFormule$}%
%   {\hbox{}$\endtrivlist}  % \hbox{} evite des underfull lors d'usages sans \< et sans \commentaire.

\newcommand{\<}[1]{\newline \hspace*{-\indentationFormule}\makebox(0,0)[bl]{$#1$}\hspace*{\indentationFormule}}

\newcommand{\commentaire}[1]{\hspace*{\indentationCommentaire}\langle\hspace*{.4em}%
\begin{minipage}[t]{\largeurBoiteCommentaire}%
#1 $\rangle$\\\hbox{}% Bizarre. Pourquoi ea prend \\ ici et aussi e la ligne suivante ?
% Sans \hbox{}, il y a des underfull.
\end{minipage}\\[-1ex] % Sans ces deux \\, l'espace apres un commentaire n'est pas le meme quand
% le commentaire a plus d'une ligne.
}

\newcommand{\commentaireligne}[1]{\mbox{\mm ---#1}}
\newcommand{\sepcom}{\mbox{ }\&\hspace{.3em}\ }



%%%%%%%%%%%%%%%% Emojis and Jokes  %%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dunno}[1][]{%
\begin{tikzpicture}[baseline,x=0.8\ht\strutbox,y=0.8\ht\strutbox,line width=0.125ex,#1]
\def\arm{(-2.5,0.95) to (-2,0.95) (-1.9,1) to (-1.5,0) (-1.35,0) to (-0.8,0)};
\draw \arm;
\draw[xscale=-1] \arm;
\def\headpart{(0.6,0) arc[start angle=-40, end angle=40,x radius=0.6,y radius=0.8]};
\draw \headpart;
\draw[xscale=-1] \headpart;
\def\eye{(-0.075,0.15) .. controls (0.02,0) .. (0.075,-0.15)};
\draw[shift={(-0.3,0.8)}] \eye;
\draw[shift={(0,0.85)}] \eye;
% draw mouth
\draw (-0.1,0.2) to [out=15,in=-100] (0.4,0.95); 
\end{tikzpicture}}


\newcommand{\smilyface}{\tikz[baseline=-0.75ex,black]{
    \draw circle (2mm);
\node[fill,circle,inner sep=0.5pt] (left eye) at (135:0.8mm) {};
\node[fill,circle,inner sep=0.5pt] (right eye) at (45:0.8mm) {};
\draw (-145:0.9mm) arc (-120:-60:1.5mm);
    }
}

\newcommand{\sadface}{...}




%%%%%%%%%%%%%%% Theorems %%%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}
%\numberwithin{theorem}{section}
%\newtheorem{proposition}[theorem]{Proposition}
%\numberwithin{theorem}{section}
%\newtheorem{corollary}[theorem]{Corollary}
%\numberwithin{theorem}{section}
%\newtheorem{lemma}[theorem]{Lemma}
%\numberwithin{theorem}{section}
%
%\theoremstyle{definition}
%\newtheorem{example}{Example}
%\numberwithin{example}{section}
%\newtheorem{fact}{FACT}
%\numberwithin{fact}{section}
%\newtheorem{remark}{Remark}
%\numberwithin{remark}{section}
%\newtheorem{hypothesis}{Hypothesis}
%\numberwithin{hypothesis}{section}
%\newtheorem{definition}{Definition}
%\numberwithin{definition}{section}
%\newtheorem{assumption}{Assumption}
%
%



%%%%%%%%%%%%%%%%% Logic Symbols %%%%%%%%%%%%
\newcommand{\vrai}{\ensuremath{\mathsf{vrai}}}
%\newcommand {\vr}{\ensuremath{\mathsf{v}}}
\newcommand {\faux}{\ensuremath{\mathsf{faux}}}
\newcommand {\fa}{\ensuremath{\mathsf{f}}}
\newcommand{\non}{\neg}
\newcommand{\et}{\wedge}
%\newcommand{\etL}{\,\wedge\,}
\newcommand{\etLL}{\,\,\wedge\,\,}
\newcommand{\ou}{\vee}
\newcommand{\ouL}{\,\vee\,}
\newcommand{\ouLL}{\,\,\vee\,\,}
\newcommand{\ssi}{\Leftrightarrow}
\newcommand{\ssiL}{\,\Leftrightarrow\,}
\newcommand{\ssidef}{\,\stackrel{\mathclap{\mbox{\tiny déf}}}{\ssi}\,}
\newcommand{\ssiLL}{\,\,\Leftrightarrow\,\,}
\newcommand{\imp}{\Rightarrow}
\newcommand{\impL}{\,\Rightarrow\,}
\newcommand{\impLL}{\,\,\Rightarrow\,\,}
\newcommand{\cons}{\Leftarrow}
\newcommand{\consL}{\,\Leftarrow\,}
\newcommand{\consLL}{\,\,\Leftarrow\,\,}






%%%%%%%%%%%%%%%  Quantifiers  %%%%%%%%%%%%%%%%%%
\newcommand{\restrict}[2]{#1_{|#2}}
\newcommand{\somme}[3]{\sum_{#1}^{#2}{#3}}
\newcommand{\produit}[3]{\prod_{#1}^{#2}{#3}}
\newcommand{\integral}[4]{\int_{#1}^{#2} #3 \,#4}
\newcommand{\unionq}[3]{\bigcup_{#1}^{#2}{#3}}
\newcommand{\intersectq}[3]{\bigcap_{#1}^{#2}{#3}}


%%%%%%%%%%%%%%%%  Sets  %%%%%%%%%%%%%%%%%%%%%
\newcommand{\nat}{\mathbb{N}} 
\newcommand{\real}{\mathbb{R}}
\newcommand{\incl}{\subset}
\newcommand{\sphere}[1]{\mathbb{S}^{#1}}
\newcommand{\theset}[1]{\{ #1 \}}
\newcommand{\lipschitz}[1]{\text{\rm Lip}_{#1} }
\newcommand{\lipnorm}[1]{\norm{#1}_\textrm{Lip}}
\newcommand{\power}[1]{\pfancy\left( #1 \right)}



%%%%%%%%%%%%%%%%  Variables  %%%%%%%%%%%%%%%%%%%%
\newcommand{\loss}{\ell}
\newcommand{\afancy}{\mathcal{A}}
\newcommand{\xfancy}{\mathcal{X}}
\newcommand{\yfancy}{\mathcal{Y}}
\newcommand{\zfancy}{\mathcal{Z}}
\newcommand{\dfancy}{\mathcal{D}}
\newcommand{\efancy}{\mathcal{E}}
\newcommand{\hfancy}{\mathcal{H}}
\newcommand{\lfancy}{\mathcal{L}}
\newcommand{\ffancy}{\mathcal{F}}
\newcommand{\gfancy}{\mathcal{G}}
\newcommand{\tfancy}{\mathcal{T}}
\newcommand{\ufancy}{\mathcal{U}}
\newcommand{\wfancy}{\mathcal{W}}
\newcommand{\pfancy}{\mathcal{P}}
\newcommand{\qfancy}{\mathcal{Q}}
\newcommand{\rfancy}{\mathcal{R}}
\newcommand{\sfancy}{\mathcal{S}}
\newcommand{\kfancy}{\mathcal{K}}
\newcommand{\sigmasq}{\sigvector^2}
\newcommand{\mmatrix}{\mathbf{M}}
\newcommand{\sigmmatrix}{\bm{\Sigma}}
\newcommand{\xmatrix}{\mathbf{X}}
\newcommand{\lammatrix}{\bm{\Lambda}}
\newcommand{\zeromatrix}{\mathbf{0}}
\newcommand{\idmatrix}{\mathbf{I}}
\newcommand{\sigvector}{\bm{\sigma}}
\newcommand{\muvector}{\bm{\mu}}
\newcommand{\zvector}{\mathbf{z}}
\newcommand{\yvector}{\mathbf{y}}
\newcommand{\xvector}{\mathbf{x}}
\newcommand{\cvector}{\mathbf{c}}
\newcommand{\hvector}{\mathbf{h}}
\newcommand{\uvector}{\mathbf{u}}
\newcommand{\wvector}{\mathbf{w}}
\newcommand{\epsvector}{\bm{\epsilon}}
\newcommand{\pivector}{\bm{\pi}}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\const}{\text{Const}}
\newcommand{\fbb}{\mathbb{F}}

\newcommand{\colvec}[2]{ \begin{bmatrix}  #1 \\ #2 \end{bmatrix} }
\newcommand{\colvecdots}[2]{ \begin{bmatrix}  #1 \\ \vdots \\ #2 \end{bmatrix} }
\newcommand{\matrixtwo}[4]{\begin{bmatrix}  #1 & #2 \\ #3 & #4 \end{bmatrix}}



%%%%%%%%%%%%%%%%%%%  Operators  %%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dotproduct}[2]{\langle #1, #2 \rangle}
\newcommand{\equdef}{\stackrel{\textrm{def}}{=}}
\newcommand{\equtop}[1]{\stackrel{(#1)}{=}}
\newcommand{\sampled}{\sim}
\newcommand{\iidsampled}{\stackrel{\text{iid}}{\sim}}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\absolu}[1]{\left \lvert #1 \right \rvert}
\newcommand{\partderiv}[1]{\frac{\partial}{\partial #1}}
\newcommand{\gradient}[2]{\nabla_{#1}{#2}}





%%%%%%%%%%%%%%%%  Functions  %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unfunc}[1]{\mathbf{1}_{#1}}
\newcommand{\expon}[1]{e^{#1}}
\newcommand{\exponbig}[1]{\textnormal{exp}\left[ #1    \right]}
%\newcommand{\argmin}[2]{\underset{#1}{\text{argmin }} #2}
%\newcommand{\argmax}[2]{\underset{#1}{\text{argmax }} #2}
\newcommand{\minfunc}[2]{\underset{#1}{\text{min }} #2}
\newcommand{\supremum}[2]{\sup_{#1} #2}





%%%%%%%%%%%%%%%%  Probabilities and Statistics %%%%%%%%%%%%%%%
\newcommand{\pushf}[2]{{#1} \sharp #2}
\newcommand{\Coupling}[1]{\Gamma(#1)}
\newcommand{\wasserstein}[2]{\text{W}_{#1}(#2)}
\newcommand{\prob}[2]{\underset{#1}{\mathbb{P}}\left[#2\right]}
\newcommand{\probseul}{\mathbb{P}}
\DeclareMathOperator*{\Esp}{\mathbb{E}}
\newcommand{\expect}[2]{\Esp_{#1}\left[#2\right]}
\newcommand{\expectseul}[2]{\Esp_{#1} #2 }
\newcommand{\expecttext}[2]{\Esp_{#1}\,[#2]}

\newcommand{\variance}[2]{\underset{#1}{\mathbb{V}} \left[ #2 \right] }
\newcommand{\variancehat}[2]{\underset{#1}{\hat{\mathbb{V}}} \left[ #2 \right] }
\newcommand{\varianceseul}[2]{\underset{#1}{\mathbb{V}} \,#2  }
\newcommand{\normal}[1]{\mathcal{N}\left( #1 \right)}
\newcommand{\mprob}[1]{\mathcal{M}_+^1(#1)}
\newcommand{\kl}[2]{\mathrm{KL}(#1 \, || \, #2)}
\newcommand{\js}[2]{\mathrm{JS}(#1 \, || \, #2)}
\newcommand{\abscont}{\ll}
\newcommand{\uniform}[1]{\ufancy_{#1}}



%%%%%%%%%%%%%%%%  Formatting &  Miscellaneous  %%%%%%%%%%%%%%%
\newcommand{\listen}[1]{#1_1, \dots, #1_n}
\newcommand{\liste}[3]{#1_{#2}, \dots, #1_{#3}}
\newcommand{\crochet}[1]{\left\langle #1 \right\rangle}
\newcommand{\rouge}[1]{\textcolor{red}{#1}}
\newcommand{\bleu}[1]{\textcolor{blue}{#1}}
\newcommand{\details}[1]{ {\color{blue} #1 } }
\newcommand{\faded}[1]{ {\color{gray} #1 } }
\newcommand{\askpascal}{\rouge{ Ask Pascal }}
\newcommand{\andspace}{\quad \text{ and } \quad}
\newcommand{\wherespace}{\quad \text{ where }}
\newcommand{\unsur}[1]{\frac{1}{#1}}
\newcommand{\omet}[1]{\details{$\bullet \bullet \bullet \bullet $}}
\newcommand{\finpreuve}{\hfill $\square$}
\newcommand{\guillemets}[1]{``#1''}





%\begin{equation*}
%\setlength{\jot}{10pt}
%\begin{split}
%... & =            \\
%    & =            \\
%    & =          \\
%    & =          \\
%    & =          \\
%    & =          \\
%    & =           \\
%\end{split}
%\end{equation*}







%\begin{equation*}
%  ...  =
%\begin{cases}
%  1, & \text{ if }   \\
%  0, & \text{otherwise}
%\end{cases}       
%\end{equation*}



%\begin{deriv}
%aaa 
%\<=
%\commentaire{ blabla }
%aaa
%\<=
%\commentaire{ blabla }
%aaa
%\<=
%\commentaire{ blabla }
%aaa
%\<=
%\commentaire{ blabla }
%aaa
%\end{deriv}









\endinput
